LASSI: An LLM-based Automated Self-Correcting Pipeline for Translating Parallel Scientific Codes

This paper addresses the problem of providing a novel approach to sourcing significant training data for LLMs focused on science and engineering. In particular, a crucial challenge is sourcing parallel scientific codes in the ranges of millions to billions of codes. To tackle this problem, we propose an automated pipeline framework called LASSI, designed to translate between parallel programming languages by bootstrapping existing closed- or open-source LLMs. LASSI incorporates autonomous enhancement through self-correcting loops where errors encountered during the compilation and execution of generated code are fed back to the LLM through guided prompting for debugging and refactoring. We highlight the bi-directional translation of existing GPU benchmarks between OpenMP target offload and CUDA to validate LASSI. The results of evaluating LASSI with different application codes across four LLMs demonstrate the effectiveness of LASSI for generating executable parallel codes, with 80% of OpenMP to CUDA translations and 85% of CUDA to OpenMP translations producing the expected output. We also observe approximately 78% of OpenMP to CUDA translations and 62% of CUDA to OpenMP translations execute within 10% of or at a faster runtime than the original benchmark code in the same language.

==> archive.tex <==
\begin{comment}
\begin{equation} \label{eq:edgeweight}
\ RT Ratio = RT_{source} / RT_{translated} \
\end{equation}
\end{comment}


\begin{comment}
\begin{table*}[ht]
\caption{OpenMP to \textbf{CUDA} translated code results: \textbf{Wizard Coder} and \textbf{DeepSeek Coder v2} LLMs}
\centering
\begin{tabular}{l|ccccc|ccccc|}
\cline{2-11}
\multirow{2}{*}{}   & \multicolumn{5}{c!{\vrule width 0.5mm}}{Wizard Coder} 
                    & \multicolumn{5}{c}{DeepSeek Coder v2}
    \\ \cline{2-11} 
                    & \multicolumn{1}{c|}{\emph{RT (s)}}
                    & \multicolumn{1}{c|}{\emph{RT Ratio}}
                    & \multicolumn{1}{c|}{\emph{Sim (T)}}
                    & \multicolumn{1}{c|}{\emph{Sim (L)}} 
                    & \emph{Self-corr}
                    & \multicolumn{1}{c|}{\emph{RT (s)}}
                    & \multicolumn{1}{c|}{\emph{RT Ratio}}
                    & \multicolumn{1}{c|}{\emph{Sim (T)}}
                    & \multicolumn{1}{c|}{\emph{Sim (L)}}
                    & \emph{Self-corr} \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{matrix-rotate} 
                    & \multicolumn{1}{c|}{1.1404} 
                    & \multicolumn{1}{c|}{1.0909} 
                    & \multicolumn{1}{c|}{0.37} 
                    & \multicolumn{1}{c|}{0.61} 
                    &  0
                    & \multicolumn{1}{c|}{1.0808} 
                    & \multicolumn{1}{c|}{1.1510} 
                    & \multicolumn{1}{c|}{0.32} 
                    & \multicolumn{1}{c|}{0.64} 
                    &  0  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{jacobi} 
                    & \multicolumn{1}{c|}{0.2892} 
                    & \multicolumn{1}{c|}{2.9879} 
                    & \multicolumn{1}{c|}{0.31} 
                    & \multicolumn{1}{c|}{0.28} 
                    &  0
                    & \multicolumn{1}{c|}{0.8327} 
                    & \multicolumn{1}{c|}{1.0377} 
                    & \multicolumn{1}{c|}{0.44} 
                    & \multicolumn{1}{c|}{0.21} 
                    &  1 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{layout} 
                    & \multicolumn{1}{c|}{0.4055} 
                    & \multicolumn{1}{c|}{1.0081} 
                    & \multicolumn{1}{c|}{0.53} 
                    & \multicolumn{1}{c|}{0.53} 
                    &  0
                    & \multicolumn{1}{c|}{0.6433} 
                    & \multicolumn{1}{c|}{0.6355} 
                    & \multicolumn{1}{c|}{0.46} 
                    & \multicolumn{1}{c|}{0.51} 
                    &  0 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{atomicCost} 
                    & \multicolumn{1}{c|}{116.2879} 
                    & \multicolumn{1}{c|}{0.3777} 
                    & \multicolumn{1}{c|}{0.59} 
                    & \multicolumn{1}{c|}{0.57} 
                    &  0
                    & \multicolumn{1}{c|}{93.1467} 
                    & \multicolumn{1}{c|}{0.4715} 
                    & \multicolumn{1}{c|}{0.58} 
                    & \multicolumn{1}{c|}{0.47} 
                    &  1 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{dense-embedding} 
                    & \multicolumn{1}{c|}{0.8137} 
                    & \multicolumn{1}{c|}{0.9899} 
                    & \multicolumn{1}{c|}{0.64} 
                    & \multicolumn{1}{c|}{0.54} 
                    &  0
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  N/A \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{pathfinder} 
                    & \multicolumn{1}{c|}{0.4804} 
                    & \multicolumn{1}{c|}{1.1282} 
                    & \multicolumn{1}{c|}{0.47} 
                    & \multicolumn{1}{c|}{0.39} 
                    &  0
                    & \multicolumn{1}{c|}{0.6821} 
                    & \multicolumn{1}{c|}{0.7946} 
                    & \multicolumn{1}{c|}{0.33} 
                    & \multicolumn{1}{c|}{0.22} 
                    &  0 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{bsearch} 
                    & \multicolumn{1}{c|}{0.2706} 
                    & \multicolumn{1}{c|}{1.2095} 
                    & \multicolumn{1}{c|}{0.35} 
                    & \multicolumn{1}{c|}{0.32} 
                    &  1
                    & \multicolumn{1}{c|}{0.2675} 
                    & \multicolumn{1}{c|}{1.2236} 
                    & \multicolumn{1}{c|}{0.42} 
                    & \multicolumn{1}{c|}{0.41} 
                    &  0  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{entropy} 
                    & \multicolumn{1}{c|}{2.3551} 
                    & \multicolumn{1}{c|}{1.0144} 
                    & \multicolumn{1}{c|}{0.50} 
                    & \multicolumn{1}{c|}{0.42} 
                    &  0
                    & \multicolumn{1}{c|}{2.4239} 
                    & \multicolumn{1}{c|}{0.9856} 
                    & \multicolumn{1}{c|}{0.58} 
                    & \multicolumn{1}{c|}{0.54} 
                    &  0  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{colorwheel} 
                    & \multicolumn{1}{c|}{0.2997} 
                    & \multicolumn{1}{c|}{1.0040} 
                    & \multicolumn{1}{c|}{0.64} 
                    & \multicolumn{1}{c|}{0.41} 
                    &  2 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  7 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{randomAccess} 
                    & \multicolumn{1}{c|}{0.3588} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{0.07} 
                    & \multicolumn{1}{c|}{0.08} 
                    &  6 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  7  \\ 
                    \hline
\end{tabular}
\label{tab:openmptocuda_2}
\end{table*}
\end{comment}


\begin{comment}
\begin{table*}[ht]
\caption{CUDA to \textbf{OpenMP} translated code results: \textbf{Wizard Coder} and \textbf{DeepSeek Coder v2} LLMs}
\centering
\begin{tabular}{l|ccccc|ccccc|}
\cline{2-11}
\multirow{2}{*}{}   & \multicolumn{5}{c!{\vrule width 0.5mm}}{Wizard Coder} 
                    & \multicolumn{5}{c}{DeepSeek Coder v2}
    \\ \cline{2-11} 
                    & \multicolumn{1}{c|}{\emph{RT (s)}}
                    & \multicolumn{1}{c|}{\emph{RT Ratio}}
                    & \multicolumn{1}{c|}{\emph{Sim (T)}}
                    & \multicolumn{1}{c|}{\emph{Sim (L)}} 
                    & \emph{Self-corr}
                    & \multicolumn{1}{c|}{\emph{RT (s)}}
                    & \multicolumn{1}{c|}{\emph{RT Ratio}}
                    & \multicolumn{1}{c|}{\emph{Sim (T)}}
                    & \multicolumn{1}{c|}{\emph{Sim (L)}}
                    & \emph{Self-corr} \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{matrix-rotate} 
                    & \multicolumn{1}{c|}{0.7645} 
                    & \multicolumn{1}{c|}{1.5435} 
                    & \multicolumn{1}{c|}{0.44} 
                    & \multicolumn{1}{c|}{0.51} 
                    &  2
                    & \multicolumn{1}{c|}{11.0047} 
                    & \multicolumn{1}{c|}{0.1072} 
                    & \multicolumn{1}{c|}{0.58} 
                    & \multicolumn{1}{c|}{0.80} 
                    &  0  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{jacobi} 
                    & \multicolumn{1}{c|}{1.4433} 
                    & \multicolumn{1}{c|}{39.7252} 
                    & \multicolumn{1}{c|}{0.42} 
                    & \multicolumn{1}{c|}{0.43} 
                    &  4
                    & \multicolumn{1}{c|}{1.6659} 
                    & \multicolumn{1}{c|}{34.4171} 
                    & \multicolumn{1}{c|}{0.37} 
                    & \multicolumn{1}{c|}{0.28} 
                    &  1 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{layout} 
                    & \multicolumn{1}{c|}{0.1326} 
                    & \multicolumn{1}{c|}{1.9404} 
                    & \multicolumn{1}{c|}{0.19} 
                    & \multicolumn{1}{c|}{0.54} 
                    &  0
                    & \multicolumn{1}{c|}{0.1639} 
                    & \multicolumn{1}{c|}{1.5699} 
                    & \multicolumn{1}{c|}{0.19} 
                    & \multicolumn{1}{c|}{0.47} 
                    &  2 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{atomicCost} 
                    & \multicolumn{1}{c|}{35.8374} 
                    & \multicolumn{1}{c|}{1.2591} 
                    & \multicolumn{1}{c|}{0.37} 
                    & \multicolumn{1}{c|}{0.23} 
                    &  1
                    & \multicolumn{1}{c|}{0.6805} 
                    & \multicolumn{1}{c|}{66.3104} 
                    & \multicolumn{1}{c|}{0.54} 
                    & \multicolumn{1}{c|}{0.46} 
                    &  1 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{dense-embedding} 
                    & \multicolumn{1}{c|}{56.6443} 
                    & \multicolumn{1}{c|}{1.0090} 
                    & \multicolumn{1}{c|}{0.54} 
                    & \multicolumn{1}{c|}{0.44} 
                    &  0
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  7 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{pathfinder} 
                    & \multicolumn{1}{c|}{0.3914} 
                    & \multicolumn{1}{c|}{1.8539} 
                    & \multicolumn{1}{c|}{0.26} 
                    & \multicolumn{1}{c|}{0.15} 
                    &  0
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  7 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{bsearch} 
                    & \multicolumn{1}{c|}{0.0158} 
                    & \multicolumn{1}{c|}{0.8861} 
                    & \multicolumn{1}{c|}{0.37} 
                    & \multicolumn{1}{c|}{0.41} 
                    &  1
                    & \multicolumn{1}{c|}{0.0048} 
                    & \multicolumn{1}{c|}{2.9167} 
                    & \multicolumn{1}{c|}{0.38} 
                    & \multicolumn{1}{c|}{0.42} 
                    &  2  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{entropy} 
                    & \multicolumn{1}{c|}{3.9525} 
                    & \multicolumn{1}{c|}{0.8763} 
                    & \multicolumn{1}{c|}{0.70} 
                    & \multicolumn{1}{c|}{0.60} 
                    &  0
                    & \multicolumn{1}{c|}{7.8830} 
                    & \multicolumn{1}{c|}{0.4394} 
                    & \multicolumn{1}{c|}{0.63} 
                    & \multicolumn{1}{c|}{0.48} 
                    &  1  \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{colorwheel} 
                    & \multicolumn{1}{c|}{0.0046} 
                    & \multicolumn{1}{c|}{0.6957} 
                    & \multicolumn{1}{c|}{0.67} 
                    & \multicolumn{1}{c|}{0.44} 
                    &  1
                    & \multicolumn{1}{c|}{0.0146} 
                    & \multicolumn{1}{c|}{0.2192} 
                    & \multicolumn{1}{c|}{0.73} 
                    & \multicolumn{1}{c|}{0.63} 
                    &  2 \\ 
                    \hline
                    \multicolumn{1}{|p{2cm}|}{randomAccess} 
                    & \multicolumn{1}{c|}{8.8987} 
                    & \multicolumn{1}{c|}{0.8896} 
                    & \multicolumn{1}{c|}{0.59} 
                    & \multicolumn{1}{c|}{0.49} 
                    &  1
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    & \multicolumn{1}{c|}{N/A} 
                    &  9 \\ 
                    \hline
\end{tabular}
\label{tab:cudatoopenmp_2}
\end{table*}
\end{comment}

==> reviewer_feedback.tex <==

SUBMISSION: 4
TITLE: LASSI: An LLM-based Automated Self-Correcting Pipeline for Translating Parallel Scientific Codes


----------------------- \textbf{REVIEW 1} ---------------------

----------- Overall evaluation -----------
SCORE: 1 (weak accept)

This paper presents LASSI, a framework aimed at automating the correction of scientific codes generated by LLMs. Overall, this paper presents a promising approach to automating the generation of parallel scientific codes using LLMs, and is a step in the right direction. However, the paper does not touch on the large body of work and existing method doing the same thing: Chain of Thoughts (CoTs), Graph of Thoughts (GoTs) etc.

Positive Aspects:

- Robust Pipeline: The automated self-correcting pipeline that LASSI employs can useful in testing different models.

- Practical Applications: The results presented, particularly the successful translation between OpenMP and CUDA, demonstrate aspect of the practical applicability of LASSI.


Areas for Improvement:

[mtd] In the following, there are suggestions on *future work* that we are already considering -- and we intentionally limited sharing too much detail on future work, so that consideration should remain in play in how we address these comments. [/mtd]

- Performance and Correctness Metrics: While the paper mentions that future work will focus on correctness and performance, a more detailed analysis in the current study would have been beneficial. Including specific examples of performance improvements and correctness checks would provide a clearer picture of LASSI’s capabilities.

[mtd] I think this is a interesting and significant effort that lends itself to a separate study as future work, so a detailed analysis is still beyond the scope of the current work. Maybe we can extend our mention for future work with more comment and expectation for challenges. [/mtd]

- Error Handling: The current approach to halting the translation process upon encountering errors is practical but could be improved. Implementing a more sophisticated error recovery mechanism could enhance the efficiency of the pipeline and reduce manual intervention.

- Detailed Case Studies: Providing in-depth case studies or examples of how LASSI handles complex translations and optimizations would enrich the paper.

[mtd] Again, complex translations and, especially, translations + code optimization is beyond the scope of demonstrating the baseline approach. However, we could specify more clearly how the architecture of LASSI enables many opportunities for extensions to advanced scenarios, including energy efficiencies, sequence-to-parallel (S2P) refactoring, performance optimization, and more. [/mtd]

- Scalability Testing: While the paper addresses the need for generating millions to billions of codes, additional testing on scalability and performance under large-scale scenarios would strengthen the argument for LASSI’s applicability in real-world settings.

[mtd] We could call this out as future work, and possibly refer to early testing from Yiheng re: enhancements to keep LASSI from getting "stuck" during self-correcting iterations. [/mtd]

- Comparing to, and discussing existing body of work as mentioned above: CoTs, GoTs, etc.

[mtd] I don't want to make the claim that LASSI is an *alternative* to CoTs, GoTs, and other prompt engineering approaches because we can incorporate these (and other) prompt engineering techniques into LASSI. So, LASSI is a framework to implement any prompt engineering method along with self-correction, so is really a 'next step' beyond CoT, GoTs, etc. and not a direct comparison. See comment in document where we could add a note about this. [/mtd]



----------------------- \textbf{REVIEW 2} ---------------------

----------- Overall evaluation -----------
SCORE: 0 (borderline paper)

The paper presents an automated pipeline to generate large quantity of synthetic code in various parallel programming languages to enable training on science LLMs such as AuroraGPT. Experimental results demonstrate the effectiveness of the code generation

Strengths
- The proposed pipeline has been designed to be agnostic to the underlying LLM. Moreover, experiments have been performed with multiple LLMs to demonstrate this feature.
- The pipeline presents a technique to self-correct compile and runtime errors by adding the errors to the context and prompting LLM to fix the errors.

Weaknesses
- It is not clear whether the performance of the generated code is due to the proposed techniques of providing the syntax guide as context, appropriate prompting and self correcting or it is because the considered LLMs have already been exposed to enough of CUDA or openMP code. This can be evaluated using two methods: (a) Not providing the syntax guide into the context and simply asking the LLM to perform the conversion and comparing the performance against the scenario where the syntax guide is provided in the context. (b) Performing translation to a language that does not have enough data (not sure which one this would be, but one way to determine would be to see for which language the LLMs perform the poorest when the syntax guide is not provided).
- One of the claims of the papers is that they address the issue of lower resource utilization in the synthetic parallel code by "carefully crafted prompts imbued with contextual knowledge and tailored programming expectations". From the prompts, it is unclear where this is happening. Moreover, the LASSI pipeline does not have any check to ensure this (for example, another module in the pipeline that check how many threads are being used, etc.). Finally, in the evaluation none of the metrics are explicitly evaluating this claim.

[mtd] The first comment re: "performance" -- Our intention is to suggest that it is through the context and self-correction that we can "coax" the LLM, that is not already exposed enough on CUDA or OpenMP, into better performance of generating better code. Our future work (i.e., currently in progress) of demonstrating a significantly reduced performance with NO CONTEXT follows exactly their recommendation with evaluating (a)  ---- and, I am confident that we can be ready to show this during the presentation at Cluster in September (but not for this revision). [/mtd]

[mtd] Re: second comment on claim of address lower resource utilization --- I need to review this claim because I don't think it should be presented as a claim that should require an evaluation metric.  Maybe just clarifying or simplifying the statement would be sufficient. ----- 

I don't see this claim made following this reviewer's interpretation -- In related works, we highlight Nichols et al. and then differentiate our work with theirs by simply saying we use CONTEXT and they DID NOT.
[/mtd]



----------------------- \textbf{REVIEW 3} ---------------------

----------- Overall evaluation -----------
SCORE: 1 (weak accept)

## Strengths

The generation of parallel scientific codes through LLM is an interesting topic and is relevant to the workshop.

## Weaknesses

- Code complexity seems very simple.
- Discussion on how different programming models would produce different quality of code by the LLM is missing.

## Detailed Comments
- A quick glance at the HeCBench repository shows that most codes there are extremely simple, with 100-200 lines of code and everything contained in the main function. The complexity of the code would be an important factor in the study, and therefore, the authors should mention the types of code, complexity, nested structures, etc.

- A discussion on How this approach can be transferred to real code would significantly motivate the work and increase its impact.

- How do different programming models such as OpenMP, CUDA, HPI, and SYCL determine the complexity of code generation and parallelization? Are there any specific code features between these models that help or restrict the model's accuracy in generating good code?

[mtd] Minimal complexity in our source code examples is intentional and known. So, maybe we need to increase our comments toward justifying this design at this stage. Future work would address all of these comments. [/mtd]



----------------------- \textbf{REVIEW 4} ---------------------

----------- Overall evaluation -----------
SCORE: 2 (accept)

The authors propose LASSI for translating parallel scientific codes, particularly between OpenMP and CUDA. Key contributions include the integration of the feedback from compilation and execution errors to create a self-correcting system capable of generating executable parallel scientific codes.The paper reports that about 78\% of OpenMP to CUDA translations and 62\% of CUDA to OpenMP translations are within 10\% of or faster than the original codes from the HeCBench suite. Authors may need to avoid the dependency in prompt chains w/ self-correcting loops.
